Secure and Efficient Group Handover Protocol in 5G Non-Terrestrial Networks

The growing low-Earth orbit (LEO) satellite constellations have become an essential part of the fifth-generation (5G) non-terrestrial network (NTN) market. These satellites can enable direct-to-cell connectivity for mobile devices and support various applications with ubiquitous coverage for 5G and beyond networks. However, satellite-based NTNs bring several challenges to the 5G handover protocol design. The high mobility of satellites can lead to signaling storms and security compromises during handovers. This paper addresses these challenges by proposing a secure and efficient group handover protocol. The protocol's effectiveness is evaluated on a custom discrete-event simulator and compared against the baseline 5G handover scheme. The simulator is made publicly available.

==> configure/copyright.tex <==
% Placeholders for submission
% Copyright
\renewcommand\footnotetextcopyrightpermission[1]{} % removes footnote with conference info
\setcopyright{none}

\settopmatter{printacmref=false, printccs=false, printfolios=false}
% DOI
\acmDOI{}

% ISBN
\acmISBN{}

%Conference
%\acmConference{ConfAbbr}
%\acmYear{2021}
%\copyrightyear{}

%---------------------------------------------------------------------------
% When accepted we get this info from the publisher

% \copyrightyear{2020} 
% \acmYear{2020} 
% \setcopyright{acmlicensed}\acmConference[MSWiM '20]{23rd International ACM Conference on Modeling, Analysis and Simulation of Wireless and Mobile Systems}{November 16--20, 2020}{Alicante, Spain}
% \acmBooktitle{23rd International ACM Conference on Modeling, Analysis and Simulation of Wireless and Mobile Systems (MSWiM '20), November 16--20, 2020, Alicante, Spain}
% \acmPrice{15.00}
% \acmDOI{10.1145/3416010.3423215}
% \acmISBN{978-1-4503-8117-8/20/11}
% % Authors, replace the red X's with your assigned DOI string during the rightsreview eform process.
% 
\settopmatter{printacmref=false}


==> content/3-background.tex <==
%\section{Background}
%\label{sec:background}

==> content/7-discussion.tex <==
\section{Discussion and Future Work}
\label{sec:discussion}






==> content/ccs-and-keywords.tex <==
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10003033.10003106.10003119.10011661</concept_id>
<concept_desc>Networks~Wireless local area networks</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10003033.10003058.10003065</concept_id>
<concept_desc>Networks~Wireless access points, base stations and infrastructure</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10003033.10003079</concept_id>
<concept_desc>Networks~Network performance evaluation</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10010583.10010588.10011669</concept_id>
<concept_desc>Hardware~Wireless devices</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Networks~Wireless local area networks}
\ccsdesc[500]{Networks~Wireless access points, base stations and infrastructure}
\ccsdesc[500]{Networks~Network performance evaluation}
\ccsdesc[500]{Hardware~Wireless devices}

\keywords{WiFi; 802.11;
frame aggregation;
aggregated MAC protocol data unit;
A-MPDU length;
optimal algorithms; 
performance evaluation;
}



==> content/macros.tex <==
% Thu Aug  5 10:39:56 EDT 2021

% It's good to use a macro for the system name because it often changes
% the name of the system so it can be easily changed
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}
\newcommand{\name}{SystemName\xspace} 
\newcommand{\bak}{block ACK\xspace} 
\newcommand{\baks}{block ACKs\xspace} 
\newcommand{\evfactors}{environmental factors\xspace} 
% \newcommand{\Name}{WiTAG}
% \newcommand{\name}{SystemName\xspace} 
% \newcommand{\witag}{WiTAG\xspace} 
%\newcommand{\tag}{WiTAG\xspace}  

% These are used to highlight changes and/or suggested changes

% todo macro used to highlight things that need changing
\newcommand{\todo}[1]{\textcolor{red}{\textbf{#1}}}
% \newcommand{\todo}[1]{}

% \newcommand{\oldtext}[1]{\textcolor{cyan}{\st{#1}}}
\newcommand{\oldtext}[1]{\textcolor{cyan}{#1}}
% \newcommand{\oldtext}[1]{}

\newcommand{\newtext}[1]{\textcolor{blue}{#1}}
% \newcommand{\newtext}[1]{#1}

% \newcommand{\name}{c{WiCom}}

\newcommand{\tofix}{\textcolor{olive}}
%\newcommand{\tofix}[1]{#1}


\newcommand{\AMPDU}{A-MPDU}
\newcommand{\DurAMPDU}{Dur_{al}}
\newcommand{\DurMessageLen}{Dur_{ml}}
\newcommand{\DurOverhead}{Dur_{overhead}}

\newcommand{\MessageLen}{ml}
\newcommand{\Length}{al}
\newcommand{\MessageRepeat}{r}
\newcommand{\NumMessages}{n}
\newcommand{\ProbOverlapWeighted}{P_{o}}
\newcommand{\Accuracy}{A}
\newcommand{\TimeDelay}{T_{d}}
\newcommand{\MaxAMPDULen}{L}
\newcommand{\ProbOverlapAMPDU}{P_{ol}}
\newcommand{\FrequencyAMPDU}{F_{l}}




